Don't Trust ChatGPT when Your Question is not in English: A Study of Multilingual Abilities and Types of LLMs

Large Language Models (LLMs) have demonstrated exceptional natural language understanding abilities and have excelled in a variety of natural language processing (NLP)tasks in recent years. Despite the fact that most LLMs are trained predominantly in English, multiple studies have demonstrated their comparative performance in many other languages. However, fundamental questions persist regarding how LLMs acquire their multi-lingual abilities and how performance varies across different languages. These inquiries are crucial for the study of LLMs since users and researchers often come from diverse language backgrounds, potentially influencing their utilization and interpretation of LLMs' results. In this work, we propose a systematic way of qualifying the performance disparities of LLMs under multilingual settings. We investigate the phenomenon of across-language generalizations in LLMs, wherein insufficient multi-lingual training data leads to advanced multi-lingual capabilities. To accomplish this, we employ a novel back-translation-based prompting method. The results show that GPT exhibits highly translating-like behaviour in multilingual settings.

==> TE-Similarities.tex <==
\begin{table*}[t]
\centering\vspace{-.2cm}
\resizebox{1\textwidth}{!}{%
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{|l|l|cccccc|cccccc|}
\hline
TE task                                                                      &                                                                        & \multicolumn{6}{c|}{Unigram similarity}                                                                                                                               & \multicolumn{6}{c|}{Bert similarity}                                                                                                                               \\ \hline
Common Sense Reasoning                              & language                                                               & \multicolumn{1}{l|}{En}      & \multicolumn{1}{l|}{Fr}       & \multicolumn{1}{l|}{De}      & \multicolumn{1}{l|}{Es}       & \multicolumn{1}{l|}{Ja}       & Zh      & \multicolumn{1}{l|}{En}      & \multicolumn{1}{l|}{Fr}      & \multicolumn{1}{l|}{De}       & \multicolumn{1}{l|}{Es}       & \multicolumn{1}{l|}{Ja}     & Zh     \\ \cline{2-14} 
                                                                             & En                                                                     & \multicolumn{1}{l|}{--}    & \multicolumn{1}{l|}{0.597}   & \multicolumn{1}{l|}{\textbf{0.601}}  & \multicolumn{1}{l|}{0.598}   & \multicolumn{1}{l|}{0.554}   & 0.555  & \multicolumn{1}{l|}{--}    & \multicolumn{1}{l|}{0.871}  & \multicolumn{1}{l|}{0.882}   & \multicolumn{1}{l|}{\textbf{0.886}}   & \multicolumn{1}{l|}{0.839} & 0.863 \\ \cline{2-14} 
                                                                             & Fr                                                                     & \multicolumn{1}{l|}{0.597}  & \multicolumn{1}{l|}{--}     & \multicolumn{1}{l|}{0.585}  & \multicolumn{1}{l|}{\textbf{0.605}}   & \multicolumn{1}{l|}{0.537}   & 0.541  & \multicolumn{1}{l|}{\textbf{0.871}}  & \multicolumn{1}{l|}{--}    & \multicolumn{1}{l|}{0.857}   & \multicolumn{1}{l|}{0.864}   & \multicolumn{1}{l|}{0.822} & 0.852 \\ \cline{2-14} 
                                                                             & De                                                                     & \multicolumn{1}{l|}{\textbf{0.601}}  & \multicolumn{1}{l|}{0.585}   & \multicolumn{1}{l|}{--}    & \multicolumn{1}{l|}{0.587}   & \multicolumn{1}{l|}{0.546}   & 0.562  & \multicolumn{1}{l|}{\textbf{0.882}}  & \multicolumn{1}{l|}{0.857}  & \multicolumn{1}{l|}{--}     & \multicolumn{1}{l|}{0.868}   & \multicolumn{1}{l|}{0.850} & 0.872 \\ \cline{2-14} 
                                                                             & Es                                                                     & \multicolumn{1}{l|}{0.598}  & \multicolumn{1}{l|}{\textbf{0.605}}   & \multicolumn{1}{l|}{0.587}  & \multicolumn{1}{l|}{--}     & \multicolumn{1}{l|}{0.536}   & 0.564  & \multicolumn{1}{l|}{\textbf{0.886}}  & \multicolumn{1}{l|}{0.864}  & \multicolumn{1}{l|}{0.868}   & \multicolumn{1}{l|}{--}     & \multicolumn{1}{l|}{0.828} & 0.866 \\ \cline{2-14} 
                                                                             & Ja                                                                     & \multicolumn{1}{l|}{0.554}  & \multicolumn{1}{l|}{0.537}   & \multicolumn{1}{l|}{0.546}  & \multicolumn{1}{l|}{0.536}   & \multicolumn{1}{l|}{--}     & \textbf{0.562}  & \multicolumn{1}{l|}{0.839}  & \multicolumn{1}{l|}{0.822}  & \multicolumn{1}{l|}{\textbf{0.850}}   & \multicolumn{1}{l|}{0.828}   & \multicolumn{1}{l|}{--}   & 0.848 \\ \cline{2-14} 
                                                                             & Zh                                                                     & \multicolumn{1}{l|}{0.555}  & \multicolumn{1}{l|}{0.541}   & \multicolumn{1}{l|}{0.562}  & \multicolumn{1}{l|}{\textbf{0.564}}   & \multicolumn{1}{l|}{0.562}   & --    & \multicolumn{1}{l|}{0.863}  & \multicolumn{1}{l|}{0.852}  & \multicolumn{1}{l|}{\textbf{0.872}}   & \multicolumn{1}{l|}{0.866}   & \multicolumn{1}{l|}{0.848} & --   \\ \cline{2-14} 
                                                                             & \begin{tabular}[c]{@{}l@{}}Average\\ Similarity to non En\end{tabular} & \multicolumn{1}{l|}{\textbf{0.581}}  & \multicolumn{1}{l|}{0.567}   & \multicolumn{1}{l|}{0.570}  & \multicolumn{1}{l|}{0.573}   & \multicolumn{1}{l|}{0.545}   & 0.557  & \multicolumn{1}{l|}{\textbf{0.868}}  & \multicolumn{1}{l|}{0.849}  & \multicolumn{1}{l|}{0.862}   & \multicolumn{1}{l|}{0.857}   & \multicolumn{1}{l|}{0.837} & 0.860 \\ \hline
Math Reasoning                                         & En                                                                     & \multicolumn{1}{l|}{--}    & \multicolumn{1}{l|}{0.794}   & \multicolumn{1}{l|}{0.788}  & \multicolumn{1}{l|}{\textbf{0.801}}   & \multicolumn{1}{l|}{0.709}   & 0.749  & \multicolumn{1}{l|}{--}    & \multicolumn{1}{l|}{0.947}  & \multicolumn{1}{l|}{0.937}   & \multicolumn{1}{l|}{\textbf{0.948}}   & \multicolumn{1}{l|}{0.907} & 0.905 \\ \cline{2-14} 
                                                                             & Fr                                                                     & \multicolumn{1}{l|}{0.794}  & \multicolumn{1}{l|}{--}     & \multicolumn{1}{l|}{0.776}  & \multicolumn{1}{l|}{\textbf{0.807}}   & \multicolumn{1}{l|}{0.698}   & 0.740  & \multicolumn{1}{l|}{\textbf{0.947}}  & \multicolumn{1}{l|}{--}    & \multicolumn{1}{l|}{0.933}   & \multicolumn{1}{l|}{\textbf{0.947}}   & \multicolumn{1}{l|}{0.905} & 0.912 \\ \cline{2-14} 
                                                                             & De                                                                     & \multicolumn{1}{l|}{0.788}  & \multicolumn{1}{l|}{0.776}   & \multicolumn{1}{l|}{--}    & \multicolumn{1}{l|}{\textbf{0.790}}   & \multicolumn{1}{l|}{0.711}   & 0.736  & \multicolumn{1}{l|}{0.937}  & \multicolumn{1}{l|}{0.933}  & \multicolumn{1}{l|}{--}     & \multicolumn{1}{l|}{\textbf{0.940}}   & \multicolumn{1}{l|}{0.910} & 0.902 \\ \cline{2-14} 
                                                                             & Es                                                                     & \multicolumn{1}{l|}{0.801}  & \multicolumn{1}{l|}{\textbf{0.807}}   & \multicolumn{1}{l|}{0.790}  & \multicolumn{1}{l|}{--}     & \multicolumn{1}{l|}{0.712}   & 0.744  & \multicolumn{1}{l|}{\textbf{0.948}}  & \multicolumn{1}{l|}{0.947}  & \multicolumn{1}{l|}{0.940}   & \multicolumn{1}{l|}{--}     & \multicolumn{1}{l|}{0.901} & 0.912 \\ \cline{2-14} 
                                                                             & Ja                                                                     & \multicolumn{1}{l|}{0.709}  & \multicolumn{1}{l|}{0.698}   & \multicolumn{1}{l|}{0.711}  & \multicolumn{1}{l|}{0.712}   & \multicolumn{1}{l|}{--}     & \textbf{0.733}  & \multicolumn{1}{l|}{0.907}  & \multicolumn{1}{l|}{0.905}  & \multicolumn{1}{l|}{\textbf{0.910}}   & \multicolumn{1}{l|}{0.901}   & \multicolumn{1}{l|}{--}   & 0.902 \\ \cline{2-14} 
                                                                             & Zh                                                                     & \multicolumn{1}{l|}{\textbf{0.749}}  & \multicolumn{1}{l|}{0.740}   & \multicolumn{1}{l|}{0.736}  & \multicolumn{1}{l|}{0.744}   & \multicolumn{1}{l|}{0.733}   & --    & \multicolumn{1}{l|}{0.905}  & \multicolumn{1}{l|}{\textbf{0.912}}  & \multicolumn{1}{l|}{0.902}   & \multicolumn{1}{l|}{\textbf{0.912}}   & \multicolumn{1}{l|}{0.902} & --   \\ \cline{2-14} 
                                                                             & \begin{tabular}[c]{@{}l@{}}Average\\ Similarity to non En\end{tabular} & \multicolumn{1}{l|}{\textbf{0.768}}  & \multicolumn{1}{l|}{0.755}   & \multicolumn{1}{l|}{0.753}  & \multicolumn{1}{l|}{0.763}   & \multicolumn{1}{l|}{0.714}   & 0.738  & \multicolumn{1}{l|}{\textbf{0.929}}  & \multicolumn{1}{l|}{0.924}  & \multicolumn{1}{l|}{0.921}   & \multicolumn{1}{l|}{0.925}   & \multicolumn{1}{l|}{0.905} & 0.907 \\ \hline
{\begin{tabular}[c]{@{}l@{}}Knowledge \\ Access\end{tabular}} & En                                                                     & \multicolumn{1}{l|}{--}    & \multicolumn{1}{l|}{0.656}   & \multicolumn{1}{l|}{0.639}  & \multicolumn{1}{l|}{\textbf{0.658}}   & \multicolumn{1}{l|}{0.584}   & 0.586  & \multicolumn{1}{l|}{--}    & \multicolumn{1}{l|}{\textbf{0.928}}  & \multicolumn{1}{l|}{0.916}   & \multicolumn{1}{l|}{0.925}   & \multicolumn{1}{l|}{0.883} & 0.858 \\ \cline{2-14} 
                                                                             & Fr                                                                     & \multicolumn{1}{l|}{0.656}  & \multicolumn{1}{l|}{--}     & \multicolumn{1}{l|}{0.651}  & \multicolumn{1}{l|}{\textbf{0.661}}   & \multicolumn{1}{l|}{0.584}   & 0.596  & \multicolumn{1}{l|}{\textbf{0.928}}  & \multicolumn{1}{l|}{--}    & \multicolumn{1}{l|}{0.926}   & \multicolumn{1}{l|}{0.922}   & \multicolumn{1}{l|}{0.888} & 0.868 \\ \cline{2-14} 
                                                                             & De                                                                     & \multicolumn{1}{l|}{0.639}  & \multicolumn{1}{l|}{\textbf{0.651}}   & \multicolumn{1}{l|}{--}    & \multicolumn{1}{l|}{0.639}   & \multicolumn{1}{l|}{0.597}   & 0.598  & \multicolumn{1}{l|}{0.916}  & \multicolumn{1}{l|}{\textbf{0.926}}  & \multicolumn{1}{l|}{--}     & \multicolumn{1}{l|}{0.903}   & \multicolumn{1}{l|}{0.878} & 0.864 \\ \cline{2-14} 
                                                                             & Es                                                                     & \multicolumn{1}{l|}{0.658}  & \multicolumn{1}{l|}{\textbf{0.661}}   & \multicolumn{1}{l|}{0.639}  & \multicolumn{1}{l|}{--}     & \multicolumn{1}{l|}{0.578}   & 0.567  & \multicolumn{1}{l|}{\textbf{0.925}}  & \multicolumn{1}{l|}{0.922}  & \multicolumn{1}{l|}{0.903}   & \multicolumn{1}{l|}{--}     & \multicolumn{1}{l|}{0.883} & 0.848 \\ \cline{2-14} 
                                                                             & Ja                                                                     & \multicolumn{1}{l|}{0.584}  & \multicolumn{1}{l|}{0.584}   & \multicolumn{1}{l|}{\textbf{0.597}}  & \multicolumn{1}{l|}{0.578}   & \multicolumn{1}{l|}{--}     & 0.567  & \multicolumn{1}{l|}{0.883}  & \multicolumn{1}{l|}{\textbf{0.888}}  & \multicolumn{1}{l|}{0.878}   & \multicolumn{1}{l|}{0.883}   & \multicolumn{1}{l|}{--}   & 0.864 \\ \cline{2-14} 
                                                                             & Zh                                                                     & \multicolumn{1}{l|}{0.586}  & \multicolumn{1}{l|}{0.596}   & \multicolumn{1}{l|}{\textbf{0.598}}  & \multicolumn{1}{l|}{0.567}   & \multicolumn{1}{l|}{0.567}   & --    & \multicolumn{1}{l|}{0.858}  & \multicolumn{1}{l|}{\textbf{0.868}}  & \multicolumn{1}{l|}{0.864}   & \multicolumn{1}{l|}{0.848}   & \multicolumn{1}{l|}{0.864} & --   \\ \cline{2-14} 
                                                                             & \begin{tabular}[c]{@{}l@{}}Average\\ Similarity to non En\end{tabular} & \multicolumn{1}{l|}{\textbf{0.624}} & \multicolumn{1}{l|}{0.623} & \multicolumn{1}{l|}{0.621} & \multicolumn{1}{l|}{0.611} & \multicolumn{1}{l|}{0.581} & 0.582 & \multicolumn{1}{l|}{\textbf{0.902}} & \multicolumn{1}{l|}{0.901} & \multicolumn{1}{l|}{0.893} & \multicolumn{1}{l|}{0.889} & \multicolumn{1}{l|}{0.878} & 0.861 \\ \hline
\end{tabular}
}%
\caption{Similarities for explanations of TE tasks.}   % {\bf DROP}}
\label{table:performance}
\end{table*}

